Network Error Logging: HTTP Archive Analysis

Network Error Logging helps web server operators detect operational problems in real-time to provide fast and reliable services. HTTP Archive provides detail information of historical data on HTTP requests. This paper leverages the data and provides a long term analysis of Network Error Logging deployment. The deployment raised from 0 to 11.73 % (almost 2,250,000 unique domains) since 2019. Current deployment is dominated by Cloudflare. Although we observed different policies, the default settings prevail. Third party collectors emerge raising the diversity needed to gather sound data. Even so, many service deploy self-hosted services. Moreover, we identify potentially malicious adversaries deploy collectors on randomly-generated domains and shortened URLs.

==> Makefile <==
# Encoding: utf-8
# Libor Polčák

# Bibliography file
BIBLIO = biblio.bib



# TeX files
TEX_FILES = $(shell ls *.tex) \
            $(BIBLIO)

FIGURES = $(shell grep '\includegraphics' *.tex | sed "s/.*{//" | sed "s/}//g" | sort | uniq | tr "\n\r" "  ")


LATEX = pdflatex
BIBTEX = bibtex
LATEX_FLAGS   =
BIBTEX_FLAGS  =

all: pdf

pdf: main.pdf


%.pdf: %.tex $(TEX_FILES) $(FIGURES)
	$(LATEX) $(LATEX_FLAGS) $(basename $<)
	$(BIBTEX) $(BIBTEX_FLAGS) $(basename $<)
	$(LATEX) $(LATEX_FLAGS) $(basename $<)
	$(LATEX) $(LATEX_FLAGS) $(basename $<)

ps: main.ps

%.ps: %.pdf
	pdftops $< $@

plain: main.txt

%.txt: %.tex ${TEX_FILES}
	cat $< | sed 's/\\ref{[^}]\+}/900/g' | tr -d "\r" | detex | awk '/./ {printf("%s ", $$0); odst=1} /^$$/ {if (odst == 1) {printf "\n\n"; odst=0}} END {printf "\n"}' | sed "s/ \+/ /g" | sed "s/ $$//" | sed "s/ ,/,/g" | sed "s/ \././g" > $@

fig/%-svg.pdf: fig/%.svg
	inkscape $< --export-type=pdf --export-filename=$@

fig/%-dot.pdf: fig/%.dot
	dot -Tpdf -Gmargin=0 -o $@ $<

fig/%-circo.pdf: fig/%.dot
	circo -Tpdf -Gmargin=0 -o $@ $<

fig/%-msc.svg: fig/%.msc
	mscgen -T svg -i $< -o $@

fig/%-msc.pdf: fig/%-msc.svg
	inkscape $< --export-type=pdf --export-filename=$@

fig/%-plot.pdf: fig/%.gp fig/%*.data
	gnuplot < $<

clean:
	rm -f *.dvi *.log  *.aux *.blg *.ist *.nlg *.nls *.nlo *.bbl

cleanall: clean
	rm -f *.dvi *.log *.aux *.tex.backup *.sty.backup
	rm -f *.blg *.bbl *.toc *.out $(NAME).tar.gz
	rm -f main.pdf main.ps

printfilenames:
	@echo "Tex:" "$(TEX_FILES)"
	@echo "Figures:" "$(FIGURES)"

arxiv.zip: $(TEX_FILES) $(FIGURES) main.bbl
	zip arxiv.zip $^

